A Forward-Inverse Dynamic Game Framework for Enhanced Multi-Agent Trajectory Planning

This paper studies feedback Nash equilibrium (FBNE) seeking for multi-agent trajectory planning in nonlinear dynamical systems with unknown agents' objectives and state-dependent inter-agent coupling. While dynamic game theory provides a principled framework for such problems, existing approaches typically assume fully rational agents with known objectives or rely on fixed regularization, limiting their ability to capture bounded rationality and spatially varying interaction intensity in safety-critical settings. To this end, we propose a KL-regularized dynamic game with a state-dependent weight that adaptively balances optimality and behavioral priors. To infer unknown cost parameters from demonstrated behaviors, we develop a context-aware inverse game module based on maximum-entropy inverse reinforcement learning with physics-informed regularization, ensuring structural consistency with the forward game. We establish per-iteration well-posedness of the regularized local game and show that the adaptive weighting function remains Lipschitz continuous under bounded nominal-trajectory updates. Numerical simulations and multi-robot experiments on cooperative navigation and merging scenarios validate the effectiveness of the proposed framework.

==> jmlr_coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We hereby submit a manuscript entitled ``\red{Distributed Stochastic Bilevel Optimization: Improved Complexity and Heterogeneity Analysis}'' by \red{Youcheng Niu, Jinming Xu, Ying Sun, Yan Huang and Li Chai}, for possible publication at the \emph{Journal of Machine Learning Research}.

Our manuscript studies \red{a class of nonconvex-stro nngly-convex distributed stochastic bilevel optimization (DSBO) problems with personalized inner-level objectives, which has recently gained increasing popularity in distributed machine learning. We propose a new loopless personalized distributed algorithm that leverages iterative approximation techniques to respectively track the inner-level solutions and Hessian-inverse matrices without relying on additional computation loops for hypergradient estimation. In contrast to most existing works, we theoretically provide a novel characterization on the heterogeneity of hypergradients among nodes for DSBO problems and establish a sublinear rate that shows the clear dependence of the convergence performance on network connectivity, sampling variances and node heterogeneity. Moreover, we eliminate the  heterogeneity by employing gradient tracking schemes. To our knowledge, this is the first study to explicitly characterize the heterogeneity as well as its influence on convergence performance in DSBO problems. Furthermore, our result achieves a computational complexity of $O(\epsilon^{-2})$ to an $\epsilon$-sationary point, which outperforms the state-of-the-art works by an order of $O(\log(\epsilon^{-1}))$.}

% with extra compensation steps controlling the impact of the approximation bias on the convergence.
% Numerical experiments are provided to verify the  effectiveness of the proposed algorithm. 
% which is important because of \red{A, B, and C}.
%
%This paper extends our work of \red{Conference Paper} by addressing \red{X, Y, and Z additional points}.

We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item \red{Martin Jaggi, EPFL, Switzerland (martin.jaggi@epfl.ch)}
    \item \red{Shiqian Ma, Rice University (sqma@rice.edu)}
    \item \red{Lam Nguyen, IBM Research (lamnguyen.mltd@ibm.com)}
    \item \red{Zaid Harchaoui, University of Washington (zaid@uw.edu)}
%    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
\end{itemize}

Reviewers:
\begin{itemize}
    % \item  \red{Hoi-To Wai, The Chinese University of Hong Kong (htwai@se.cuhk.eduhk)}
    \item  \red{Songtao Lu, IBM Thomas J. Watson Research Center (songtaoibm@gmail.com) }
     \item \red{Saeed Ghadimi, University of Waterloo (sghadimi@uwaterloo.ca)}
    \item  \red{Qing Ling, Sun Yat-Sen University (lingqing556@mail.sysu.edu.cn) }
    \item \red{Jordan Frecon, Jean Monnet University (jordan.frecon@gmail.com)}    
    % \item \red{Olivier Fercoq, Telecom Paris (olivier.fercoq@telecom-paris.fr)}
    % \item \red{Luo Luo, Fudan University (luoluo@fudan.edu.cn)}
    \item \red{Kevin Scaman, INRIA Paris (kevin.scaman@inria.fr)}
%    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
\end{itemize}
Our submission has the following keywords: \red{distributed learning}, \red{bilevel optimization}, \red{non-convex optimization}, \red{heterogeneity analysis}, \red{gradient tracking}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the journal.

\bigskip

Sincerely,

\medskip

Jinming Xu, on behalf of the authors\\
College of Control Science and Engineering\\
Zhejiang University\\
Hangzhou, China 310007
% \red{Ying Sun (The Pennsylvania State University, USA)}\\
% \red{Yan Huang (Zhejiang University, China)} \\
% \red{Li Chai (Zhejiang University, China)}
% \red{Youcheng Niu (Zhejiang University, China)}\\
\end{document}







































